Compass Control: Multi Object Orientation Control for Text-to-Image Generation

Existing approaches for controlling text-to-image diffusion models, while powerful, do not allow for explicit 3D object-centric control, such as precise control of object orientation. In this work, we address the problem of multi-object orientation control in text-to-image diffusion models. This enables the generation of diverse multi-object scenes with precise orientation control for each object. The key idea is to condition the diffusion model with a set of orientation-aware \textbf{compass} tokens, one for each object, along with text tokens. A light-weight encoder network predicts these compass tokens taking object orientation as the input. The model is trained on a synthetic dataset of procedurally generated scenes, each containing one or two 3D assets on a plain background. However, direct training this framework results in poor orientation control as well as leads to entanglement among objects. To mitigate this, we intervene in the generation process and constrain the cross-attention maps of each compass token to its corresponding object regions. The trained model is able to achieve precise orientation control for a) complex objects not seen during training and b) multi-object scenes with more than two objects, indicating strong generalization capabilities. Further, when combined with personalization methods, our method precisely controls the orientation of the new object in diverse contexts. Our method achieves state-of-the-art orientation control and text alignment, quantified with extensive evaluations and a user study.

==> sec/HeilmeierCatechism.tex <==
\section{Heilmeier Catechism}

\subsection{What are you trying to do? Articulate your objectives using absolutely no jargon.}
- Text-to-image diffusion models can generate highly realistic and diverse images; however, they are limited to the text and 2D control. 
- We provide an additional 3D control to control the object individually pose in a disentangled manner. 
- This is highly desirable for designers and artists, as it enables them to generate complex scenes with multiple objects with precise 3D control.


\subsection{How is it done today, and what are the limits of current practice?}
- There are a few works that achieve 3D pose control in the generation. However, they are severely limited
- Object centric - Existing methods focus on editing the pose of a single object - Continuous words, zero-123
- individual training on each data distribution - neural assets -> not for generation but editing 
- multi-view - requires dense multi-view posed images of the subject to be generated in novel scenes -> cd 360, view-neti


\subsection{What is new in your approach and why do you think it will be successful?}
- Training on synthetic datasets with different viewpoints for a small set of objects
- We do not explicitly model the 3D during the generation process (cd-360, mv-edit) or condition on 3D layout (lc), but still achieve hq pose control in 
  the generation 
- We show the knowledge is already there in SD and training with a small set of categories extracts that knowledge in an interpretable form, 
  enabling generalization to novel object categories and multiple objects in scenes
- pose token for each object 
- To reduce the disentanglement, we propose a novel attention regularization during training, which attends the pose token to only the region associated 
  with the generated object category.  
- Not rely on large-scale training, small synthetic datasets with augmentations generated using a control for realistic images 


\subsection{Who cares? If you are successful, what difference will it make?}
- It provides a finer control in the scene generation process and shows there are already 3D properties existing in text-to-image models
- We have provided a novel interface to extract this 3d control, enabling a fine-grained view control in the generation process 


\subsection{Evaluations?}
We evaluate our models for scene generation with multiple objects for - pose control, scene realism and prompt consistency 
We also show our method can generate realistic compositions beating the baselines for realism and pose control
An extensive user study suggests, we can generate hq compositions and outperform all the baselines by a significant margin. 
